Conserved energies for the cubic NLS in 1-d

We consider the cubic Nonlinear Schr\"odinger Equation (NLS) as well as the modified Korteweg-de Vries (mKdV) equation in one space dimension. We prove that for each $s>-\frac12$ there exists a conserved energy which is equivalent to the $H^s$ norm of the solution. For the Korteweg-de Vries (KdV) equation there is a similar conserved energy for every $s\ge -1$.

==> shuffle.tex <==
\makeatletter
\providecommand*{\shuffle}{%
  \mathbin{\mathpalette\shuffle@{}}%
}
\newcommand*{\shuffle@}[2]{%
  % #1: math style
  % #2: unused
  \sbox0{$#1\vcenter{}$}%
  \kern .15\ht0 % side bearing
  \rlap{\vrule height .25\ht0 depth 0pt width 2.5\ht0}%
  \raise.1\ht0\hbox to 2.5\ht0{%
    \vrule height 1.75\ht0 depth -.1\ht0 width .17\ht0 %
    \hfill
    \vrule height 1.75\ht0 depth -.1\ht0 width .17\ht0 %
    \hfill
    \vrule height 1.75\ht0 depth -.1\ht0 width .17\ht0 %
  }%
  \kern .15\ht0 % side bearing
}
\def\DeclareConnection#1#2{\expandafter\gdef\csname MH@symb@#1\endcsname{\kern0.1em\tikz[baseline=0,scale=0.2,draw=symbols]{#2}\kern0.1em}}
\def\<#1>{\csname MH@symb@#1\endcsname}
\makeatother

\DeclareConnection{XY}{\draw[basic] (0,0) .. controls  (0.25,1.5) and (.75,1.5) .. (1,0);}
\DeclareConnection{XYXY}{\<XY>\<XY>} 
\DeclareConnection{XXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);}
\DeclareConnection{XYXYXY}{\<XY>\<XY>\<XY>} 
\DeclareConnection{XYXXYY}{\<XY>\<XXYY>} 

\DeclareConnection{XXXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);}
\DeclareConnection{XXYXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (0.25,0) .. controls  (1.06,2) and (3.18,2) .. (4,0);}
\DeclareConnection{XXXXYYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);
\draw[basic] (-.5,0) .. controls (.5,2.5) and (2.5 ,2.5) .. (3.5,0); 
}
\DeclareConnection{XXXYXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (0.25,0) .. controls  (1.06,2) and (3.18,2) .. (4,0);
\draw[basic] (-.25,0) .. controls (1,2.5) and (3.25 ,2.5) .. (4.5,0); 
}
\DeclareConnection{XXXYYXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (2.75,0) .. controls  (3,1) and (3.5,1) .. (3.75,0);
\draw[basic] (0,0) .. controls (1.06,2.5) and (3.18 ,2.5) .. (4.25,0); 
}
\DeclareConnection{XXYXXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.5,0) .. controls  (2.75,1) and (3.25,1) .. (3.5,0);
\draw[basic] (2.25,0) .. controls  (2.62,1.5) and (3.38,1.5) .. (3.75,0);
\draw[basic] (0,0) .. controls (1.06,2.5) and (3.18 ,2.5) .. (4.25,0); 
}


\DeclareConnection{XXYXYXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (3.5,0) .. controls  (3.75,1) and (4.25,1) .. (4.5,0);
\draw[basic] (.5,0) .. controls (1.5,2) and (4 ,2) .. (5,0); 
}

% 10 Variables
\DeclareConnection{XXXXXYYYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);
\draw[basic] (-.5,0) .. controls (.5,2.5) and (2.5 ,2.5) .. (3.5,0); 
\draw[basic] (-1,0) .. controls (0.25,3) and (2.75 ,3) .. (4,0); 
}

\DeclareConnection{XXXXYXYYYY}
{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (0.25,0) .. controls  (1.06,2) and (3.18,2) .. (4,0);
\draw[basic] (-.25,0) .. controls (1,2.5) and (3.25 ,2.5) .. (4.5,0); 
\draw[basic] (-.75,0) .. controls (.5 ,3) and (3.75,3) ..(5,0); 
}

\DeclareConnection{XXXXYYXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (2.75,0) .. controls  (3,1) and (3.5,1) .. (3.75,0);
\draw[basic] (0,0) .. controls (1.06,2.5) and (3.18 ,2.5) .. (4.25,0); 
\draw[basic] (-.5,0) .. controls (.5,3) and (4.25,3)..(4.75,0); 
}

\DeclareConnection{XXXXYYYXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);
\draw[basic] (3.25,0) .. controls (3.5,1) and (4,1) ..(4.25,0);
\draw[basic] (-0.5,0) .. controls (.75   ,3) and (3.5 ,3) ..(4.75,0);
}


\DeclareConnection{XXXYXXYYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.5,0) .. controls  (2.75,1) and (3.25,1) .. (3.5,0);
\draw[basic] (2.25,0) .. controls  (2.62,1.5) and (3.38,1.5) .. (3.75,0);
\draw[basic] (0,0) .. controls (1.06,2.5) and (3.18 ,2.5) .. (4.25,0); 
\draw[basic] (-.5,0) .. controls (.5,3) and (4.25,3)..(4.75,0); 
}
%432

\DeclareConnection{XXXYXYXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (3.5,0) .. controls  (3.75,1) and (4.25,1) .. (4.5,0);
\draw[basic] (.5,0) .. controls (1.5,2) and (4 ,2) .. (5,0); 
\draw[basic] (0,0) .. controls (1.25,2.5) and (4.25,2.5) .. (5.5,0);
}

%144
\DeclareConnection{XXXYXYYXYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (0.25,0) .. controls  (1.06,2) and (3.18,2) .. (4,0);
\draw[basic] (4.25,0) .. controls ( 4.5,1)  and (5,1) .. (5.25,0);
\draw[basic] (-.25,0) .. controls  (1.25,3) and (4.25 ,3) .. (5.75,0);
}



%48
\DeclareConnection{XXXYYXYXYY}{
\draw[basic] (-1.5,0) .. controls (-1.25,1) and (-.75,1) .. (-.5,0);
\draw[basic] (-1.75,0) .. controls (-1.38 ,1.5) and (-.62,1.5) ..(-.25,0);
\draw[basic] (0,0) .. controls (.25,1) and (.75,1) .. (1,0);
\draw[basic] (1.25,0) .. controls (1.5,1) and (2,1) .. (2.25,0);
\draw[basic] (-2,0) .. controls (-1.75,2.5) and (1.5 ,2.5) ..(2.75,0); 
}  


%288
\DeclareConnection{XXYXXXYYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (0.5,0) .. controls  (1,1.5) and (2,1.5) .. (2.5,0);
\draw[basic] (0,0) .. controls  (1,2) and (2,2) .. (3,0);
\draw[basic] (-1.25,0) .. controls (-1,1) and (-.5,1) .. (-.25,0);
\draw[basic] (-1.75,0) .. controls (-.5,3) and (2.25,3) .. (3.5,0);}

%144 
\DeclareConnection{XXYXXYXYYY}{\draw[basic] (1,0) .. controls  (1.25,1) and (1.75,1) .. (2,0);\draw[basic] (2.25,0) .. controls  (2.5,1) and (3,1) .. (3.25,0);
\draw[basic] (0.25,0) .. controls  (1.06,2) and (3.18,2) .. (4,0);
\draw[basic] (-1,0) .. controls (-.75,1) and (-.25,1) ..(0,0);
\draw[basic] (-1.5,0) .. controls ( 0 ,3) and ( 3 ,3) .. (4.5,0); 
}

%48 
\DeclareConnection{XXYXXYYXYY}{
\draw[basic] (1.25,0) .. controls (1.5,1) and (2,1) .. (2.25,0);
\draw[basic] (3,0) .. controls (3.25,1) and (3.75,1) .. (4,0);
\draw[basic] (2.75,0) .. controls (3.12 ,1.5) and (3.88,1.5) ..(4.25,0);
\draw[basic] (4.5,0) .. controls (4.75,1) and (5.25,1) .. (5.5,0);
\draw[basic] (.75,0) .. controls (1.25,2.5) and (4.75 ,2.5) ..(6,0); 
 } 


\DeclareConnection{XXYXYXXYYY}{
\draw[basic] (0,0) .. controls (.25,1) and (.75,1) .. (1,0);
\draw[basic] (1.25,0) .. controls (1.5,1) and (2,1) .. (2.25,0);
\draw[basic] (3,0) .. controls (3.25,1) and (3.75,1) .. (4,0);
\draw[basic] (2.75,0) .. controls (3.12 ,1.5) and (3.88,1.5) ..(4.25,0);
\draw[basic] (-.5,0) .. controls (.25,2.5) and (3.5 ,2.5) ..(4.75,0); 
}  


\DeclareConnection{XXYXYXYXYY}{
\draw[basic] (0,0) .. controls (.25,1) and (.75,1) .. (1,0);
\draw[basic] (1.25,0) .. controls (1.5,1) and (2,1) .. (2.25,0);
\draw[basic] (2.5,0) .. controls (2.75,1) and (3.25,1) .. (3.5,0);
\draw[basic] (3.75,0) .. controls (4,1) and (4.5,1) .. (4.75,0);
\draw[basic] (-.5,0) .. controls (.5,2) and (4.25,2) .. (5.25,0); 
} 


\makeatother

